Ultra-directional and high-efficiency $\mu$LEDs via gradient index filled micro-Horn collimators

Micro-LEDs ($\mu$LEDs) are poised to transform AR/VR, display, and optical communication technologies, but they are currently hindered by low light extraction efficiency and non-directional emission. Our study introduces an innovative approach using a descending index multilayer anti-reflection coating combined with a horn collimator structure atop the $\mu$LED pixel. This design leverages the propagation of light outside the critical angle to enhance both the directionality and extraction efficiency of emitted light. By implementing either discrete or continuous refractive index gradients within the horn, we achieve a dramatic tenfold increase in light extraction within a $\pm$15$^\circ$ cone, with an overall light extraction efficiency reaching approximately 80%, where 31% of the power is concentrated within this narrow cone. This performance surpasses that of an optimized SiO2 half-ellipsoidal lens, which diameter and height is 24X and 26X larger than the pixel width respectively, while our design only slightly increases the device height and expands the final light escape surface to 3 times and roughly 4 times the pixel width respectively. Such efficiency, directionality enhancement, and compactness make this solution particularly suitable for high-resolution, densely packed $\mu$LED arrays, promising advancements in high-performance, miniaturized display systems.

==> 3_methods.tex <==
\subsection{Simulation}

All waveoptical simulations are performed using lumerical FDTD simulation software while using open source available material data. 
